Carnegie Supernova Project-II: Extending the Near-Infrared Hubble Diagram for Type Ia Supernovae to $z\sim0.1$

The Carnegie Supernova Project-II (CSP-II) was an NSF-funded, four-year program to obtain optical and near-infrared observations of a "Cosmology" sample of $\sim100$ Type Ia supernovae located in the smooth Hubble flow ($0.03 \lesssim z \lesssim 0.10$). Light curves were also obtained of a "Physics" sample composed of 90 nearby Type Ia supernovae at $z \leq 0.04$ selected for near-infrared spectroscopic time-series observations. The primary emphasis of the CSP-II is to use the combination of optical and near-infrared photometry to achieve a distance precision of better than 5%. In this paper, details of the supernova sample, the observational strategy, and the characteristics of the photometric data are provided. In a companion paper, the near-infrared spectroscopy component of the project is presented.

==> v5.0 arXiv/Tables/Tab1.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lccllccc}
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablewidth{0pt}
\tablecaption{CSP-II SNe~Ia\label{tab:allsne}}
\tablehead{
\colhead{SN Name} &
\colhead{R.A. (2000)} &
\colhead{Dec. (2000)} &
\colhead{Host Galaxy} &
\colhead{$z_{\rm{helio}}$\tablenotemark{a}} &
\colhead{Discovery\tablenotemark{b}} &
\colhead{Classification\tablenotemark{b}} &
\colhead{Subsample\tablenotemark{c}}
}
\startdata
ASASSN-14ad                     &   12:40:11.10   &   +18:03:32.80   &   KUG 1237+183                     &   $0.0264$                    &   ASASSN   &  (14)       &   P     \\
ASASSN-14hp                     &   21:30:31.42   &   -70:38:34.35   &   2MASX J21303015-7038489          &   $0.0389$                    &   ASASSN   &   CSP      &   C     \\
ASASSN-14hr                     &   01:50:41.27   &   -14:31:06.37   &   2MASX J01504127-1431032          &   $0.0336$                    &   ASASSN   &   CSP      &   C   \\
ASASSN-14hu                     &   06:43:26.92   &   -69:38:14.70   &   ESO 058- G 012                   &   $0.0216$\tablenotemark{d}   &   ASASSN   &   CSP      &   P     \\
ASASSN-14jc                     &   07:35:35.29   &   -62:46:12.64   &   2MASX J07353554-6246099          &   $0.0113$                    &   ASASSN   &   PESSTO   &   P     \\
ASASSN-14jg                     &   23:33:13.90   &   -60:34:11.50   &   2MASX J23331223-6034201          &   $0.0148$                    &   ASASSN   &   LCOGT    &   P     \\
ASASSN-14jz                     &   18:44:44.34   &   -52:48:05.48   &   GALEXASC J184443.33-524819.2     &   $0.0158$\tablenotemark{d}   &   ASASSN   &   PESSTO   &        \\
ASASSN-14kd                     &   22:53:24.95   &   +04:47:57.30   &   2MASX J22532475+0447583          &   $0.0242$\tablenotemark{d}    &   ASASSN   &   PESSTO   &        \\
ASASSN-14kq                     &   23:45:15.51   &   -29:47:01.14   &   2MASX J23451480-2947009          &   $0.0336$                    &   ASASSN   &   CSP      &   C   \\
ASASSN-14lo                     &   11:51:53.11   &   +18:32:29.00   &   UGC 06837                        &   $0.0199$                    &   ASASSN   &   LCOGT    &   P     \\
ASASSN-14lp                     &   12:45:09.10   &   -00:27:32.49   &   NGC 4666                         &   $0.0051$                    &   ASASSN   &   ASASSN   &   P     \\
ASASSN-14lq                     &   22:57:19.41   &   -20:58:00.76   &   2MASX J22571481-2058014          &   $0.0262$                    &   ASASSN   &  (15)       &   P     \\
ASASSN-14lt                     &   03:11:02.54   &   -13:06:38.76   &   IC 0299                          &   $0.0320$                    &   ASASSN   &   Asiago   &   C   \\
ASASSN-14lw                     &   01:06:49.17   &   -46:58:59.96   &   GALEXASC J010647.95-465904.1     &   $0.0209$\tablenotemark{d}   &   ASASSN   &   CSP      &   P     \\
ASASSN-14me                     &   01:26:40.08   &   -57:59:49.31   &   ESO 113- G 047                   &   $0.0178$\tablenotemark{d}    &   ASASSN   &   ASASSN   &   P     \\
ASASSN-14mf                     &   00:04:54.46   &   -32:26:14.63   &   GALEXASC J000454.54-322615.3     &   $0.0311$                    &   ASASSN   &   ASASSN   &   C   \\
ASASSN-14mw                     &   01:41:25.16   &   -65:37:01.26   &   AM 0139-655 NED02                &   $0.0274$                  &   ASASSN,OGLE   &   ASASSN   &   C,P   \\
ASASSN-14my                     &   11:38:29.98   &   -08:58:35.79   &   NGC 3774                         &   $0.0205$                &   ASASSN,PS1   &   CSP      &   P     \\
ASASSN-15aj                     &   10:52:53.26   &   -32:55:34.86   &   NGC 3449                         &   $0.0109$                    &   ASASSN   &   CSP      &   P     \\
ASASSN-15al                     &   04:57:49.63   &   -21:35:34.11   &   GALEXASC J045749.46-213526.3     &   $0.0338$\tablenotemark{d}   &   ASASSN,Gaia   &   PESSTO   &   C     \\
ASASSN-15as                     &   09:39:16.55   &   +06:25:48.53   &   SDSS J093916.69+062551.1         &   $0.0286$\tablenotemark{d}   &   ASASSN   &   CSP      &   C,P   \\
ASASSN-15ba                     &   14:04:55.09   &   +08:55:14.53   &   SDSS J140455.12+085514.0         &   $0.0231$                    &   ASASSN,CRTS   &   CfA      &   P     \\
ASASSN-15be                     &   02:52:46.39   &   -34:18:52.52   &   GALEXASC J025245.83-341850.6     &   $0.0219$                    &   ASASSN   &   ASASSN   &   P     \\
ASASSN-15bm                     &   15:05:51.58   &   -05:37:37.05   &   LCRS B150313.2-052600            &   $0.0208$\tablenotemark{d}   &   ASASSN   &   ASASSN   &   P     \\
ASASSN-15cb                     &   12:39:50.23   &   +03:47:49.77   &   VCC 1810                         &   $0.0400$                    &   ASASSN,PS1   &   PESSTO   &   C     \\
ASASSN-15cd                     &   09 59 14.75   &   +12 59 20.53   &   CGCG 064-017                     &   $0.0344$                    &   ASASSN   &   PESSTO   &   C     \\
ASASSN-15da                     &   05:23:51.88   &   -24:42:08.38   &   2MASX J05235106-2442201          &   $0.055$\tablenotemark{e}    &   ASASSN   &   ASASSN   &   C     \\
ASASSN-15db                     &   15:46:58.69   &   +17:53:02.55   &   NGC 5996                         &   $0.0110$                    &   ASASSN   &  (16)       &        \\
ASASSN-15dd                     &   15:43:59.07   &   +19:12:40.74   &   CGCG 107-031                     &   $0.0244$                    &   ASASSN   &   ASASSN   &        \\
ASASSN-15eb                     &   08:06:07.40   &   -22:33:48.86   &   ESO 561- G 012                   &   $0.0165$                    &   ASASSN   &   SMT      &   P     \\
ASASSN-15fr                     &   09:20:20.44   &   -07:38:26.78   &   2MASX J09202045-0738229          &   $0.0334$                    &   ASASSN   &   Asiago   &   C,P   \\
ASASSN-15ga                     &   12:59:27.29   &   +14:10:15.79   &   NGC 4866                         &   $0.0066$                    &   ASASSN   &  (17)       &   P     \\
ASASSN-15go                     &   06:11:30.50   &   -16:29:03.52   &   2MASX J06113048-1629085          &   $0.0189$                    &   ASASSN   &   SMT      &   P     \\
ASASSN-15gr                     &   06:45:20.58   &   -34:53:38.11   &   ESO 366- G 015                   &   $0.0243$\tablenotemark{d}   &   ASASSN   &   PESSTO   &   P     \\
ASASSN-15hf                     &   10:29:31.00   &   -35:15:35.60   &   ESO 375- G 041                   &   $0.0062$                    &   ASASSN   &   PESSTO   &   P     \\
ASASSN-15hg                     &   09:53:48.62   &   +09:11:37.78   &   CGCG 063-098                     &   $0.0298$                    &   ASASSN   &  (18)       &   C   \\
ASASSN-15hx                     &   13:43:16.69   &   -31:33:21.55   &   GALEXASC J134316.80-313318.2     &   $0.0083$\tablenotemark{d}    &   ASASSN   &   PESSTO   &   P     \\
PSN J13471211-2422171           &   13:47:12.11   &   -24:22:17.10   &   ESO 509- G 108                   &   $0.0199$                    &   BOSS,ASASSN           &   CSP      &   P     \\
SN2014ao                        &   08:34:33.32   &   -02:32:36.10   &   NGC 2615                         &   $0.0141$                    &   LOSS,ASASSN   &   Asiago   &   P     \\
SN2014I                         &   05:42:19.80   &   -25:32:39.90   &   ESO 487-G36                      &   $0.0300$                    &   BOSS,ASASSN   &   SMT      &   C,P   \\
SN2014eg                        &   02:45:09.27   &   -55:44:16.90   &   ESO 154- G 010                   &   $0.0186$                    &  (1),ASASSN   &   PESSTO   &   P     \\
\hline
CSS111231:145323+025743 (SN2011jt)  &   14:53:23.01   &   +02:57:43.10   &   CGCG 048-051                     &   $0.0278$                    &   CRTS     &   LOSS     &   P     \\
CSS120224:145405+220541 (SN2012aq)  &   14:54:05.13   &   +22:05:40.60   &   SDSS J145405.13+220540.7         &   $0.052$\tablenotemark{e}    &   CRTS     &   Asiago   &   C     \\
CSS120301:162036-102738 (SN2012ar)  &   16:20:36.02   &   -10:27:38.30   &   2MASX J16203650-1028061          &   $0.0283$                    &   CRTS     &   Asiago   &   C,P \\
CSS120325:123816-150632         &   12:38:16.19   &   -15:06:32.15   &   anonymous                        &   $0.0972$\tablenotemark{d}   &   CRTS     &   CRTS     &   C   \\
CSS121114:090202+101800         &   09:02:02.34   &   +10:18:00.10   &   SDSS J090202.18+101759.7         &   $0.0371$                    &   CRTS     &  (19)       &   C     \\
CSS130215:033841+101827 (SN2013ad) &   03:38:41.04   &   +10:18:27.22   &   anonymous                        &   $0.0363$\tablenotemark{d}   &   CRTS     &   CSP      &   C     \\
CSS130303:105206-133424         &   10:52:06.06   &   -13:34:24.70   &   GALEXASC J105206.27-133420.2     &   $0.0789$\tablenotemark{d}   &   CRTS     &   PESSTO   &   C     \\
CSS130315:115252-185920 (SN2013as)  &   11:52:52.34   &   -18:59:19.90   &   anonymous                        &   $0.0685$\tablenotemark{d}   &   CRTS     &   PESSTO   &   C     \\
CSS131031:095508+064831         &   09:55:08.22   &   +06:48:31.40   &   SDSS J095510.00+064830.3         &   $0.0777$                    &   CRTS     &   PESSTO   &   C     \\
CSS140126:120307-010132         &   12:03:06.88   &   -01:01:31.70   &   SDSS J120306.76-010132.4         &   $0.0772$\tablenotemark{d}   &   CRTS     &   PESSTO   &   C     \\
CSS140218:095739+123318         &   09:57:39.11   &   +12:33:17.70   &   SDSS J095738.31+123308.5         &   $0.0773$\tablenotemark{d}   &   CRTS     &   PESSTO   &   C     \\
CSS140914:010107-101840         &   01:01:07.04   &   -10:18:39.90   &   anonymous                        &   $0.03$\tablenotemark{e}     &   CRTS     &   PESSTO   &  C     \\
CSS140925:162946+083831 (SN2014dl)  &   16:29:46.09   &   +08:38:30.60   &   UGC 10414                        &   $0.0330$                    &   CRTS     &   CSP      &   C   \\
CSS150214:140955+173155 (SN2015bo) &   14:09:55.13   &   +17:31:55.60   &   NGC 5490                         &   $0.0162$                    &   CRTS     &   PESSTO   &   P     \\
SNhunt161 (SN2012hl)    &   00:50:17.76   &   +24:31:52.20   &   CSS J005017.69+243154.4          &   $0.0332$\tablenotemark{d}    &   CRTS     &  (20)       &        \\
SNhunt177 (SN2013az)   &   05:39:52.13   &   -40:30:28.10   &   ESO 306-016                      &   $0.0373$                    &   CRTS     &   PESSTO   &   C     \\
SNhunt178 (SN2013bc)  &   13:10:21.31   &   -07:10:24.10   &   IC 4209                          &   $0.0225$                    &   CRTS     &   CSP      &   P     \\
SNhunt188 (SN2013bz)   &   13:26:51.32   &   -10:01:32.20   &   2MASX J13265081-1001263          &   $0.0192$                    &   CRTS     &  (21)       &   P     \\
SNhunt229 (SN2014D)    &   12:10:36.76   &   +18:49:35.40   &   UGC 07170                        &   $0.0082$                    &   CRTS,PS1     &   CSP      &   P     \\
SNhunt281 (SN2015bp)  &   15:05:30.07   &   +01:38:02.40   &   NGC 5839                         &   $0.0041$                    &   CRTS     &  (22)       &   P     \\
SSS111226:125715-172401 (SN2011jn)   &   12:57:14.79   &   -17:24:00.50   &   2MASX J12571157-1724344          &   $0.0475$                    &   CRTS     &  (23)       &   C     \\
MASTER OT J093953.18+165516.4 &   09:39:53.18   &   +16:55:16.40   &   CGCG 092-024                     &   $0.0478$                    &   MASTER,CRTS   &   PESSTO   &   C     \\
SN2014du  &   02:26:23.31   &   +27:39:34.80   &   UGC 01899                        &   $0.0325$                    &   ISSP,CRTS     &   Asiago   &   C,P   \\
\hline
KISS13j (SN2013Y)               &   12:09:39.70   &   +16:12:14.30   &   SDSS J120939.62+161212.2         &   $0.0766$                    &   KISS     &   KISS     &   C     \\
KISS13l (SN2013al)              &   11:14:54.07   &   +29:35:06.00   &   SDSS J111454.06+293508.7         &   $0.1321$                    &   KISS     &  (24)       &   C     \\
KISS13v (SN2013ba)              &   13:52:56.63   &   +21:56:21.70   &   SDSS J135256.58+215621.1         &   $0.080$\tablenotemark{e}    &   KISS     &   KISS     &   C     \\
KISS15m                          &   12:06:00.83   &   +20:36:18.40   &   NGC 4098                         &   $0.0243$                    &   KISS,CRTS     &   CSP      &        \\
SN2015M               &   13:00:32.33   &   +27:58:41.00   &   GALEXMSC J130032.33+275842.3 ?   &   $0.0231$\tablenotemark{g} &   KISS,CRTS,PS1     &   CSP      &   P   \\
\hline
LSQ11bk                         &   04:20:44.25   &   -08:35:55.75   &   anonymous                        &   $0.0403$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ11ot                         &   05:15:48.34   &   +06:46:39.36   &   CGCG 421-013                     &   $0.0273$                    &   LSQ      &  (25)       &   C,P,L \\
LSQ11pn (SN2011jq)            &   05:16:41.54   &   +06:29:29.40   &   2MASX J05164149+0629376          &   $0.0327$                    &   LSQ      &   SNF      &   C,P,L \\
LSQ12ca                         &   05:31:03.62   &   -19:47:59.28   &   2MASX J05310364-1948063          &   $0.0994$\tablenotemark{d}   &   LSQ      &   LCOGT    &   L     \\
LSQ12agq                        &   10:17:41.67   &   -07:24:54.45   &   GALEXASC J101741.80-072452.2     &   $0.0642$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ12aor                        &   10:55:17.64   &   -14:18:01.38   &   GALEXASC J105517.85-141757.2     &   $0.0934$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ12bld                        &   13:42:44.03   &   +08:05:33.74   &   SDSS J134244.72+080531.7         &   $0.0837$                    &   LSQ      &   CSP      &   C,L   \\
LSQ12blp                        &   13:36:05.59   &   -11:37:16.87   &   LCRS B133326.3-112212            &   $0.0743$                    &   LSQ,CRTS      &   CSP      &   C,L   \\
LSQ12btn                        &   09:21:30.47   &   -09:41:29.86   &   2MASX J09213114-0941331          &   $0.0542$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ12cda                        &   13:50:02.32   &   +09:37:47.10   &   SDSS J135002.40+093755.1         &   $0.1376$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ12cdl                        &   12:53:39.96   &   -18:30:26.16   &   GALEXASC J125339.85-183025.6     &   $0.1081$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ12fuk                        &   04:58:15.88   &   -16:17:58.03   &   GALEXASC J045815.88-161800.7     &   $0.0206$\tablenotemark{d}   &   LSQ,CRTS      &   SNF      &   P,L   \\
LSQ12fvl                        &   05:00:50.04   &   -38:39:11.51   &   MCG -06-12-002                   &   $0.0560$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ12fxd                        &   05:22:17.02   &   -25:35:47.01   &   ESO 487- G 004                   &   $0.0312$                    &   LSQ,CRTS      &   PESSTO   &   C,P,L \\
LSQ12gdj                        &   23:54:43.32   &   -25:40:34.09   &   ESO 472- G 007                   &   $0.0303$                    &   LSQ      &   SNF      &   C,P,L \\
LSQ12gef                        &   01:40:33.70   &   +18:30:36.38   &   2MASX J01403375+1830406          &   $0.0642$\tablenotemark{d}   &   LSQ      &   SNF      &   L     \\
LSQ12gln                        &   05:22:59.41   &   -33:27:51.32   &   GALEXASC J052259.58-332755.3     &   $0.1021$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ12gpw                        &   03:12:58.24   &   -11:42:40.13   &   2MASX J03125885-1142402          &   $0.0506$\tablenotemark{d}   &   LSQ      &   PESSTO   &   L     \\ 
LSQ12gxj                        &   02:52:57.38   &   +01:36:24.25   &   2MASX J02525699+0136231          &   $0.0355$\tablenotemark{f}   &   LSQ      &   PESSTO   &   L     \\
LSQ12gyc                        &   02:45:50.07   &   -17:55:45.74   &   anonymous                        &   $0.0932$\tablenotemark{f}   &   LSQ      &   PESSTO   &   L     \\ 
LSQ12gzm                        &   02:40:43.61   &   -34:44:25.87   &   GALEXASC J024043.58-344425.0     &   $0.1001$\tablenotemark{d}   &   LSQ      &   PESSTO   &   L     \\
LSQ12hjm                        &   03:10:28.72   &   -16:29:37.08   &   2MASX J03102844-1629333          &   $0.0714$\tablenotemark{d}   &   LSQ      &   SNF      &   L     \\
LSQ12hno                        &   03:42:43.25   &   -02:40:09.76   &   GALEXASC J034243.43-024007.7     &   $0.0473$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ12hnr                        &   10:43:14.77   &   -08:46:40.89   &   anonymous                        &   $0.135$\tablenotemark{f}    &   LSQ      &   PESSTO   &   C,L   \\
LSQ12hvj                        &   11:07:38.62   &   -29:42:40.96   &   GALEXASC J110738.65-294235.5     &   $0.0713$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ12hxx                        &   03:19:44.23   &   -27:00:25.68   &   2MASX J03194423-2700201          &   $0.0694$                    &   LSQ      &   SNF      &   C,L   \\
LSQ12hzj                        &   09:59:12.43   &   -09:00:08.25   &   2MASX J09591230-0900095          &   $0.0334$\tablenotemark{d}   &   LSQ      &   SNF      &   C,P,L \\
LSQ12hzs                        &   04:01:53.21   &   -26:39:50.15   &   2MASXi J0401529-263947           &   $0.0721$                    &   LSQ      &   CSP      &   C,L   \\
LSQ13lq                         &   13:44:10.81   &   +03:03:43.42   &   SDSS J134410.77+030345.3         &   $0.0757$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ13pf                         &   13:48:14.35   &   -11:38:38.58   &   LCRS B134534.3-112338            &   $0.0861$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ13ry                         &   10:32:48.00   &   +04:11:51.75   &   SDSS J103247.83+041145.5         &   $0.0299$                    &   LSQ      &   CSP      &   C,P,L \\
LSQ13vy                         &   16:06:55.85   &   +03:00:15.23   &   2MASX J16065563+0300046          &   $0.0418$\tablenotemark{d}   &   LSQ      &   LCOGT    &   C,L   \\
LSQ13abo                        &   14:59:21.20   &   -17:09:09.34   &   2MASX J14592124-1709138          &   $0.0675$                    &   LSQ      &   SNF      &   C,L   \\
LSQ13aiz (SN2013cs)             &   13:15:14.81   &   -17:57:55.65   &   ESO 576- G 017                   &   $0.0092$  &   LSQ,CRTS      &  (26)       &   P,L   \\
LSQ13cwp                        &   04:03:50.65   &   -02:39:17.98   &   2MASX J04035024-0239275          &   $0.0666$   &   LSQ      &   CSP      &   C,L   \\
LSQ13dby                        &   03:26:42.84   &   -34:38:05.49   &   anonymous                        &   $0.100$\tablenotemark{e}    &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dcy                        &   04:55:16.42   &   -20:00:05.40   &   LCSB S0801P                      &   $0.0801$\tablenotemark{d}    &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dhj                        &   02:12:34.48   &   -37:20:22.81   &   GALEXMSC J021234.60-372019.1     &   $0.0935$\tablenotemark{d}    &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dkp                        &   03:10:09.97   &   -36:37:44.91   &   2MASX J03101094-3638017          &   $0.0690$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dpm                        &   10:29:08.32   &   -17:06:50.19   &   GALEXASC J102908.61-170654.2     &   $0.0509$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dqh                        &   04:22:05.90   &   -02:53:24.24   &   anonymous                        &   $0.1038$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ13dsm                        &   03:33:12.83   &   -26:12:24.02   &   APMUKS(BJ) B033105.19-262232.9   &   $0.0424$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ14q                          &   08:53:57.58   &   +17:19:38.19   &   SDSS J085357.19+171942.6         &   $0.0667$                    &   LSQ,PS1      &   PESSTO   &   C,L   \\
LSQ14ba                         &   11:01:23.01   &   -15:37:10.29   &   GALEXASC J110123.17-153706.2     &   $0.0776$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ14ie                         &   12:55:33.46   &   -32:56:40.37   &   anonymous                        &   $0.0896$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ14ip                         &   09:44:20.22   &   +04:35:52.56   &   2MASX J09442084+0435319          &   $0.0613$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14jp                         &   12:57:21.51   &   -15:47:33.42   &   2MASX J12572166-1547411          &   $0.0454$                    &   LSQ      &   CSP      &   C,L   \\
LSQ14mc                         &   09:02:13.45   &   +17:03:37.01   &   SDSS J090213.35+170335.4         &   $0.0567$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14wp                         &   10:14:05.72   &   +06:40:30.54   &   SDSS J101405.83+064032.5         &   $0.0695$\tablenotemark{d}   &   LSQ,CRTS      &   PESSTO   &   C,L   \\
LSQ14xi                         &   12:30:41.17   &   -13:46:21.91   &   2MASX J12304088-1346236          &   $0.0508$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14act                        &   15:59:44.65   &   -10:26:40.80   &   2MASX J15594429-1026396          &   $0.0591$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14age                        &   13:24:08.62   &   -13:26:26.00   &   GALEXASC J132408.58-132629.0     &   $0.0806$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ14ahc                        &   13:43:48.25   &   -32:54:35.12   &   2MASX J13434760-3254381          &   $0.0509$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ14ahm                        &   11:41:22.44   &   -12:23:57.69   &   GALEXASC J114122.65-122354.9     &   $0.0498$\tablenotemark{d}   &   LSQ,CRTS      &   PESSTO   &   C,L   \\
LSQ14ajn (SN2014ah)             &   11:55:30.88   &   +11:55:25.88   &   CGCG 068-091                     &   $0.0210$                    &   LSQ,PS1      &   Asiago   &   P,L   \\
LSQ14asu                        &   11:11:35.95   &   -21:27:59.63   &   2MASX J11113635-2127597          &   $0.0684$                    &   LSQ      &   CSP      &   C,L   \\
LSQ14auy                        &   14:28:11.30   &   -04:03:17.50   &   2MASX J14281171-0403150          &   $0.0825$                    &   LSQ      &   CSP      &   C,L   \\
LSQ14azy                        &   11:12:34.73   &   +12:04:24.83   &   2MASX J11123493+1204206          &   $0.0458$                    &   LSQ      &  (27)       &   L     \\
LSQ14bbv                        &   19:59:33.12   &   -56:59:27.84   &   2MASS J19593264-5659334          &   $0.0588$\tablenotemark{d}   &   LSQ      &   CSP      &   L     \\
LSQ14bjj                        &   14:20:49.08   &   -05:15:02.25   &   APMUKS(BJ) B141811.91-050120.8   &   $0.0812$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ14fms                        &   00:14:59.82   &   -51:12:39.54   &   2MASX J00145929-5112380          &   $0.078$\tablenotemark{d}    &   LSQ      &   CSP      &   C,L   \\
LSQ14foj                        &   00:26:34.67   &   -32:48:33.09   &   GALEXASC J002634.59-324825.5     &   $0.0461$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14fom                        &   21:59:49.73   &   -30:16:15.56   &   2MASX J21594968-3016187          &   $0.0563$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14gfb                        &   05:10:05.76   &   -36:18:43.57   &   2MASX J05100559-3618388          &   $0.0527$                    &   LSQ      &   PESSTO   &   C,L   \\
LSQ14gfn                        &   03:28:32.16   &   -04:12:14.22   &   2MASX J03283205-0412113          &   $0.1217$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ14ghv                        &   03:23:44.15   &   -31:35:03.17   &   2MASX J03234449-3135101          &   $0.0667$                    &   LSQ      &   LCOGT    &   C,L   \\
LSQ14gov                        &   04:06:01.33   &   -16:01:41.49   &   GALEXMSC J040601.67-160139.7     &   $0.0896$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ15bv                         &   10:59:47.29   &   -16:49:10.63   &   2MASX J10594717-1649070          &   $0.0689$                    &   LSQ      &  (28)       &   C,L   \\
LSQ15aae                        &   16:30:15.70   &   +05:55:58.73   &   2MASX J16301506+0555514          &   $0.0516$\tablenotemark{d}   &   LSQ      &   CSP      &   C,L   \\
LSQ15agh                        &   10:52:54.78   &   +23:27:41.65   &   2MASX J10525434+2335518          &   $0.0603$                    &   LSQ      &   CSP      &   C,L   \\
LSQ15aja                        &   17:03:08.92   &   +12:27:41.65   &   SDSS J170308.90+122741.5     &   $0.0700$\tablenotemark{d}   &   LSQ      &   PESSTO   &   C,L   \\
LSQ15alq                        &   13:09:18.56   &   -25:52:20.24   &   ESO 508- G 016                   &   $0.0471$                    &   LSQ,PS1      &   CSP      &   C,L   \\
\hline
MASTER OT J030559.89+043238.2   &   03:05:59.89   &   +04:32:38.20   &   SDSS J030559.63+043246.0         &   $0.0282$\tablenotemark{d}   &   MASTER   &   CfA      &   P     \\
\hline
OGLE-2012-SN-040                &   06:07:01.59   &   -69:21:17.10   &   2MASX J06070178-6921180          &   $0.0147$                    &   OGLE     &   PESSTO   &        \\
OGLE-2013-SN-015                &   02:02:21.56   &   -65:44:08.66   &   2MASX J02022241-6544090          &   $0.0890$\tablenotemark{d}   &   OGLE     &   CSP      &   C     \\
OGLE-2013-SN-109                &   01:46:09.34   &   -67:28:00.10   &   2MASX J01460987-6727579          &   $0.0868$\tablenotemark{d}    &   OGLE     &   PESSTO   &   C     \\
OGLE-2013-SN-118                &   05:14:47.50   &   -66:50:29.10   &   2MASX J05144615-6650292          &   $0.0750$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
OGLE-2013-SN-123                &   05:58:30.38   &   -63:33:38.30   &   2MASX J05583036-6333386          &   $0.0614$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
OGLE-2013-SN-126                &   04:19:47.21   &   -63:43:22.04   &   anonymous                        &   $0.0597$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
OGLE-2013-SN-148                &   06:38:06.97   &   -75:43:37.21   &   2MASX J06380745-7543288          &   $0.0404$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
OGLE-2014-SN-019                &   06:13:48.04   &   -67:55:15.00   &   2MASX J06134795-6755146          &   $0.0359$                    &   OGLE     &   PESSTO   &   C     \\
OGLE-2014-SN-021                &   05:48:23.49   &   -66:47:29.70   &   anonymous                        &   $0.0422$\tablenotemark{d}   &   OGLE     &   SMT      &   C     \\
OGLE-2014-SN-107                &   00:42:28.75   &   -64:45:51.00   &   APMUKS(BJ) B004021.02-650219.5   &   $0.0664$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
OGLE-2014-SN-141                &   05:37:18.64   &   -75:43:17.00   &   2MASX J05371898-7543157          &   $0.0625$\tablenotemark{d}   &   OGLE     &   PESSTO   &   C     \\
SN2015F   &   07:36:15.76   &   -69:30:23.00   &   NGC 2442                         &   $0.0049$                    &   (2),OGLE     &   PESSTO   &   P     \\
\hline
PS1-13eao                       &   03:29:56.35   &   -28:46:17.70   &   ESO 418- G 007                   &   $0.0378$                    &   PS1      &   PESSTO   &   C     \\
PS1-14ra                        &   14:41:28.44   &   +09:25:58.70   &   IC 1044                          &   $0.0281$                    &   PS1      &   PESSTO   &   C,P   \\
PS1-14rx                        &   12:46:53.35   &   +14:47:50.10   &   SDSS J124653.32+144748.4         &   $0.0666$                    &   PS1      &   PESSTO   &   C     \\
PS1-14xw                        &   16:52:57.93   &   +02:23:36.50   &   NGC 6240                         &   $0.0245$                    &   PS1      &   PESSTO   &        \\
PS15sv                          &   16:13:11.74   &   +01:35:31.10   &   GALEXASC J161311.68+013532.2     &   $0.0333$\tablenotemark{d}   &   PS1      &   PESSTO   &   C,P   \\
SN2013ct     &   01:12:54.92   &   +00:58:45.70   &   NGC 428                          &   $0.0038$                    &   BOSS,PS1     &   CSP      &   P     \\
SN2013gy    &   03:42:16.88   &   -04:43:18.48   &   NGC 1418                         &   $0.0140$                    &   LOSS,PS1,CRTS   &   Asiago   &   P     \\
\hline
PTF11pbp (SN2011hb)             &   23:27:55.52   &   +08:46:45.00   &   NGC 7674                         &   $0.0289$                    &   PTF,CRTS      &   PTF      &   C,P   \\
PTF11ppn                        &   21:35:21.93   &   +26:56:04.70   &   2MASX J21352164+2656051          &   $0.0673$\tablenotemark{d}   &   PTF      &   PTF      &   C     \\
PTF11pra (SN2011hk)              &   02:18:45.81   &   -06:38:31.00   &   NGC 881                          &   $0.0176$                    &   PTF      &   PTF      &        \\
PTF11qnr (SN2011im)     &   22:44:25.45   &   -00:10:02.00   &   NGC 7364                         &   $0.0162$                    &   PTF      &   PTF      &   P     \\
iPTF13ez                        &   12:09:51.30   &   +19:47:15.70   &   SDSS J120951.25+194716.5         &   $0.0436$                    &   iPTF     &   iPTF     &   C   \\
iPTF13anh                       &   13:06:50.45   &   +15:34:32.36   &   SDSS J130650.44+153432.7         &   $0.0614$\tablenotemark{d}   &   iPTF,CRTS     &   iPTF     &   C     \\
iPTF13duj                       &   21:13:44.78   &   +13:34:33.10   &   NGC 7042                         &   $0.0170$                    &   iPTF     &   LCOGT    &   P     \\
iPTF13dwl                       &   21:16:49.05   &   +12:00:50.80   &   GALEXASC J211648.97+120052.8     &   $0.0875$\tablenotemark{d}   &   iPTF     &   iPTF     &   C     \\
iPTF13dym                       &   23:24:30.19   &   +14:39:04.00   &   SDSS J232430.20+143903.6         &   $0.0422$                    &   iPTF     &   iPTF     &   C     \\
iPTF13ebh                       &   02:21:59.98   &   +33:16:13.70   &   NGC 0890                         &   $0.0133$                    &   iPTF     &   CSP      &   P     \\
iPTF13efe                       &   08:43:39.30   &   +16:10:37.30   &   SDSS J084339.26+161037.5         &   $0.0751$\tablenotemark{d}   &   iPTF,CRTS     &   iPTF     &   C     \\
iPTF14fpg (SN2014dk)            &   00:28:12.00   &   +07:09:43.50   &   SDSS J002812.09+070940.0       &   $0.034$\tablenotemark{e}   &   iPTF,PS1,CRTS     &   Asiago   &   C,P   \\
iPTF14yw (SN2014aa)             &   11:45:03.58   &   +19:58:25.40   &   NGC 3861                         &   $0.0170$                    &   iPTF     &   Asiago   &   P     \\
iPTF14w                         &   12:03:31.29   &   +02:02:34.00   &   UGC 07034                        &   $0.0189$                    &   iPTF     &   Asiago   &   P     \\
iPTF14uo                        &   13:18:57.69   &   +09:42:40.30   &   GALEXASC J131857.37+094244.0     &   $0.0913$\tablenotemark{d}   &   iPTF     &   iPTF     &   C     \\
iPTF14yy                        &   12:26:09.17   &   +09:58:44.20   &   SDSS J122608.78+095847.1         &   $0.0431$                    &   iPTF     &   iPTF     &   C   \\
iPTF14aje                       &   15:25:12.07   &   -01:48:51.50   &   SDSS J152512.43-014840.1         &   $0.0276$                    &   iPTF     &   iPTF     &   C   \\
iPTF14gnl                       &   00:23:48.33   &   -03:51:27.90   &   LCSB S0066P                      &   $0.0537$                    &   iPTF     &   iPTF     &   C     \\
\hline
ROTSE3 J123935.1+163512 (SN2012G)  &   12:39:35.10   &   +16:35:11.90   &   IC 0803 NED01                    &   $0.0258$\tablenotemark{d}   &   ROTSE-III,MASTER     &  (29)       &   P     \\
\hline
SMT J03253351-5344190            &   03:25:33.51   &   -53:44:19.00   &   anonymous                        &   $0.0592$\tablenotemark{d}   &   SMT      &   SMT      &   C     \\
\hline
SN2011iv                        &   03:38:51.34   &   -35:35:32.00   &   NGC 1404                         &   $0.0065$                    &   BOSS     &  (30)       &   P     \\
SN2011iy                        &   13:08:58.38   &   -15:31:04.00   &   NGC 4984                         &   $0.0043$                    &  (3)       &  (31)      &   P     \\
SN2011jh                        &   12:47:14.42   &   -10:03:47.30   &   NGC 4682                         &   $0.0078$                    &  (4)       &   Asiago   &   P     \\
SN2012E                         &   02:33:22.79   &   +09:35:05.60   &   NGC 975                          &   $0.0203$                    &  (5)        &   Asiago   &   P     \\
SN2012U                         &   02:06:04.33   &   -55:11:37.50   &   ESO 153- G 020                   &   $0.0197$                    &   BOSS     &  (32)       &   P     \\
SN2012ah                        &   23:25:59.63   &   -81:54:33.30   &   NGC 7637                         &   $0.0124$                    &   BOSS    &  (33)      &   P     \\
SN2012bl                        &   20:23:55.28   &   -48:21:17.30   &   ESO 234-019                      &   $0.0187$                    &   CHASE    &  (34)       &   P     \\
SN2012bo                        &   12:50:45.23   &   -14:16:08.50   &   NGC 4726                         &   $0.0254$                    &  (6)        &   Asiago   &   P     \\
SN2012fr                        &   03:33:36.10   &   -36:07:34.00   &   NGC 1365                         &   $0.0055$                    &   TAROT    &   SMT      &   P     \\
SN2012gm                        &   23:17:37.03   &   +14:00:08.90   &   NGC 7580                         &   $0.0148$                    &  (7)        &   Asiago   &   P     \\
SN2012hd                        &   01:14:07.46   &   -32:39:07.70   &   IC 1657                          &   $0.0120$                    &   BOSS     &   PESSTO   &   P     \\
SN2012hr                        &   06:21:38.46   &   -59:42:50.60   &   ESO 121- G 026                   &   $0.0076$                    &   BOSS     &   CSP      &   P     \\
SN2012ht                        &   10:53:22.75   &   +16:46:34.90   &   NGC 3447                         &   $0.0036$                    &  (8)        &  (8)        &   P     \\
SN2012id                        &   04:42:41.14   &   +18:34:59.70   &   2MASX J04424248+1835003          &   $0.0157$                    &  (9)        &   Asiago   &   P     \\
SN2012ij                        &   11:40:15.84   &   +17:27:22.20   &   CGCG 097-050                     &   $0.0110$                    &   TNTS     &  (35)       &   P     \\
SN2013E                         &   10:00:05.52   &   -34:14:01.30   &   IC 2532                          &   $0.0094$                    &   BOSS     &   CSP      &   P     \\
SN2013H                         &   09:06:30.70   &   -75:49:01.50   &   ESO 036- G 019                   &   $0.0155$                    &   BOSS     &   CSP      &   P     \\
SN2013M                         &   13:59:56.68   &   -37:51:49.40   &   ESO 325- G 043                   &   $0.0350$                    &   BOSS     &  (36)       &   C,P   \\
SN2013U                         &   10:01:12.00   &   +00:19:42.30   &   CGCG 008-023                     &   $0.0345$                    &  (10)        &   Asiago   &   C,P   \\
SN2013aa                        &   14:32:33.88   &   -44:13:27.80   &   NGC 5643                         &   $0.0040$                    &   BOSS     &  (37)       &   P     \\
SN2013aj                        &   13:54:00.68   &   -07:55:43.80   &   NGC 5339                         &   $0.0091$                    &  (11)        &  (11)        &   P     \\
SN2013ay                        &   18:42:37.86   &   -64:56:13.50   &   IC 4745                          &   $0.0157$                    &   CHASE    &   CSP      &   P     \\
SN2013cg                        &   09:26:56.77   &   -24:46:59.60   &   NGC 2891                         &   $0.0080$                    &   CHASE    &  (38)       &   P     \\
SN2013fy                        &   21:37:27.12   &   -47:01:54.80   &   ESO 287- G 040                   &   $0.0309$                    &   BOSS     &   PESSTO   &   C,P   \\
SN2013fz                        &   04:23:46.44   &   -51:35:46.30   &   NGC 1578                         &   $0.0206$                    &   BOSS     &   PESSTO   &   P     \\
SN2013gv                        &   03:09:57.31   &   +19:12:49.20   &   IC 1890                          &   $0.0341$                    &  (12)      &   Asiago   &   C,P   \\
SN2013hh                        &   11:29:04.37   &   +17:14:09.50   &   UGC 06483                        &   $0.0130$                    &   TAROT    &   SMT      &   P     \\
SN2013hn                        &   13:48:59.17   &   -30:17:26.50   &   IC 4329                          &   $0.0151$                    &  (13)       &   LCOGT    &   P     \\
SN2014Z                         &   01:44:07.99   &   -61:07:07.40   &   ESO 114- G 004                   &   $0.0213$                    &   BOSS     &   CSP      &   P     \\
SN2014at                        &   21:46:14.82   &   -46:31:21.10   &   NGC7119                          &   $0.0322$                    &  BOSS    &   PESSTO   &   C,P   \\
SN2014ba                        &   22:55:01.97   &   -39:39:34.50   &   NGC 7410                         &   $0.0058$                    &   BOSS     &  (39)       &   P     \\
SN2014bz                        &   13:56:04.19   &   -43:35:09.90   &   2MASX J13560316-4334319          &   $0.0225$                    &   TAROT    &   SMT      &        \\
SN2014dn                        &   04:17:54.27   &   -56:36:45.20   &   IC 2060                          &   $0.0222$                    &   BOSS     &   CSP      &        \\
\enddata
\tablenotetext{a}{Heliocentric redshift are
from the NASA/IPAC Extragalactic Database (NED) unless otherwise indicated.}
\tablenotetext{b}{ASASSN \citep{shappee14,holoien17}; Asiago \citep{tomasella14}; BOSS (\url{http://bosssupernova.com/}); CHASE \citep{pignata09}; 
CfA (\url{https://www.cfa.harvard.edu/supernova//RecentSN.html}); CRTS \citep{djorgovski11}; CSP (this paper); iPTF \citep{kulkarni13}; 
ISSP (\url{http://italiansupernovae.org/en/project/description.html}); Gaia \citep{altavilla12}; KISS \citep{morokuma14}; LCOGT \citep{howell14}; LOSS \citep{filippenko01}; 
LSQ \citep{baltay13}; MASTER \citep{gorbovskoy13}; OGLE \citep{wyrzykowski14}; PESSTO \citep{smartt15}; PS1 \citep{kaiser10,scolnic18}; 
PTF \citep{law09}; ROTSE-III \citep{akerlof03}; SMT \citep{scalzo17}; SNF \citep{wood-vasey04}; TAROT \citep{klotz08}; TNTS \citep{yao15}}
\tablenotetext{c}{C = ``Cosmology''; P = ``Physics''; L = ``LSQ''}
\tablenotetext{d}{Redshift measured by CSP-II}
\tablenotetext{e}{Approximate redshift derived from SN spectrum}
\tablenotetext{f}{Peter Nugent (private communication)}
\tablenotetext{g}{Redshift of Coma Cluster}
\tablerefs{
(1) \citet{kangas14}; 
(2) \citet{CBET4081}; 
(3) \citet{CBET2943}; 
(4) \citet{nakano11}; 
(5) \citet{cox12}; 
(6) \citet{itagaki12}; 
(7) \citet{rich12}; 
(8) \citet{nishiyama12}; 
(9) \citet{yusa12}; 
(10) \citet{gagliano13}; 
(11) \citet{cortini13}; 
(12) \citet{kiyota13}; 
(13) \citet{kot13}; 
(14) \citet{ATel5823}  
(15) \citet{ATel6814};  
(16) \citet{ATel7086};   
(17) \citet{ATel7333};  
(18) \citet{ATel7420};  
(19) \citet{ATel4597};  
(20) \citet{CBET3335};  
(21) \citet{CBET3507}; 
(22) \citet{ATel7251}; 
(23) \citet{CBET2963}; 
(24) \citet{CBET3438}; 
(25) \citet{ATel3826}; 
(26) \citet{ATel5067}; 
(27) \citet{ATel6080}; 
(28) \citet{ATel6952}; 
(29) \citet{CBET2983}; 
(30) \citet{CBET2940,CBET2940b}; 
(31) \citet{CBET2943b,CBET2943c}; 
(32) \citet{CBET3007}; 
(33) \citet{CBET3028}; 
(34) \citet{CBET3076}; 
(35) \citet{CBET3370}; 
(36) \citet{CBET3393}; 
(37) \citet{CBET3416}; 
(38) \citet{CBET3517}; 
(39) \citet{CBET3873}
}
%\tablenotetext{a}{La Silla-Quest Low Redshift Survey \citep{baltay13}}
%\tablenotetext{b}{Catalina Real Time Transit Survey \citep{djorgovski11}}
%\tablenotetext{c}{Intermediate Palomar Transient Factory \citep{law09,kulkarni13}}
%\tablenotetext{d}{OGLE-IV Real-Time Transient Search \citep{wyrzykowski14}}
%\tablenotetext{e}{All-Sky Automated Survey for SuperNovae \citep{holoien17}}
%\tablenotetext{f}{Pan-STARRS1 Medium Deep Survey \citep{kaiser10,scolnic17}}
%\tablenotetext{g}{Backyard Observatory Supernova Search \url{http://bosssupernova.com/}}
%\tablenotetext{h}{Kiso Supernova Survey \citep{morokuma14}}
%\tablenotetext{i}{SkyMapper Transient Survey \citep{scalzo17}}
%\tablenotetext{j}{Mobile Astronomy System of TElescope Robots \citep{gorbovskoy13}}
%\tablenotetext{k}{Italian Supernovae Search Project \url{http://italiansupernovae.org/en/project/description.html}}
%\tablenotetext{l}{\citet{kiyota13,gagliano13}}
\end{deluxetable*}
\end{longrotatetable}


==> v5.0 arXiv/Tables/Tab2.tex <==
\begin{deluxetable}{lccc}
\tabletypesize{\scriptsize}
\tablecolumns{4}
\tablewidth{0pt}
\tablecaption{CSP-II Cosmology Subsample Sources\label{tab:sources}}
\tablehead{
\colhead{Source} &
\colhead{Untargeted?} &
\colhead{\# of SNe} &
\colhead{Percentage}
}
\startdata
LSQ\tablenotemark{a}          & Yes & 60 & 48.0\% \\
CRTS\tablenotemark{b}       & Yes & 15 & 12.0\% \\
ASASSN\tablenotemark{c}      & Yes & 14 & 11.2\% \\
PTF/iPTF\tablenotemark{d}  & Yes & 12 & 9.6\% \\
OGLE\tablenotemark{e}       & Yes & 10 & 8.0\% \\
PS1\tablenotemark{f}           & Yes & 4 & 3.2\% \\
KISS\tablenotemark{g}         & Yes & 3 & 2.4\% \\
SMT\tablenotemark{h}          & Yes & 1 & 0.8\% \\
MASTER\tablenotemark{i}   & Yes & 1 & 0.8\% \\
 & & {---}{---} & {---}{---} \\
 & & 120 & 96.0\% \\
 & & & \\
 BOSS\tablenotemark{j}       & No & 3 & 2.4\% \\
%ISSP\tablenotemark{k}          & No & 1 & 0.8\% \\
Other\tablenotemark{l}         & No & 2 & 1.6\% \\
 & & {---}{---} & {---}{---} \\
 & & 5 & 4.0\% \\
\enddata
\tablenotetext{a}{La Silla-Quest Low Redshift Survey \citep{baltay13}}
\tablenotetext{b}{Catalina Real Time Transit Survey \citep{djorgovski11}}
\tablenotetext{c}{All-Sky Automated Survey for SuperNovae \citep{shappee14,holoien17}}
\tablenotetext{d}{Palomar Transient Factory \citep{law09} /Intermediate Palomar Transient Factory \citep{kulkarni13}}
\tablenotetext{e}{OGLE-IV Real-Time Transient Search \citep{wyrzykowski14}}
\tablenotetext{f}{Pan-STARRS1 Medium Deep Survey \citep{kaiser10,scolnic18}}
\tablenotetext{g}{Kiso Supernova Survey \citep{morokuma14}}
\tablenotetext{h}{SkyMapper Transient Survey \citep{scalzo17}}
\tablenotetext{i}{Mobile Astronomy System of TElescope Robots \citep{gorbovskoy13}}
\tablenotetext{j}{Backyard Observatory Supernova Search \url{http://bosssupernova.com/}}
\tablenotetext{k}{Italian Supernovae Search Project \url{http://italiansupernovae.org/en/project/description.html}}
\tablenotetext{l}{\citet{gagliano13,kiyota13}}
\end{deluxetable}

==> v5.0 arXiv/Tables/Tab3.tex <==
\begin{deluxetable}{lccc}
\tabletypesize{\scriptsize}
\tablecolumns{4}
\tablewidth{0pt}
\tablecaption{CSP-II Physics Subsample Sources\label{tab:sources_physics}}
\tablehead{
\colhead{Source} &
\colhead{Untargeted?} &
\colhead{\# of SNe} &
\colhead{Percentage}
}
\startdata
ASASSN\tablenotemark{a}      & Yes & 27 & 30.0\% \\
LSQ\tablenotemark{b}          & Yes & 9 & 10.0\% \\
CRTS\tablenotemark{c}       & Yes & 8 & 8.9\% \\
PTF/iPTF\tablenotemark{d}  & Yes & 7 & 7.8\% \\
PS1\tablenotemark{e}           & Yes & 4 & 4.4\% \\
KISS\tablenotemark{f}         & Yes & 1 & 1.1\% \\
MASTER\tablenotemark{g}   & Yes & 1 & 1.1\% \\
OGLE\tablenotemark{h}   & Yes & 1 & 1.1\% \\
ROTSE-III\tablenotemark{i}  & Yes & 1 & 1.1\%\\
 & & {---}{---} & {---}{---} \\
 & & 59 & 65.6\% \\
 & & & \\
BOSS\tablenotemark{j}       & No & 14 & 15.6\% \\
CHASE\tablenotemark{k}          & No & 3 & 3.3\% \\
TAROT\tablenotemark{l}          & No & 2 & 2.2\% \\
%LOSS\tablenotemark{k}          & No & 1 & 1.1\% \\
TNTS\tablenotemark{m}          & No & 1 & 1.1\% \\
%ISSP\tablenotemark{m}          & No & 1 & 1.1\% \\
Other\tablenotemark{n}         & No & 11 & 12.2\% \\
 & & {---}{---} & {---}{---} \\
 & & 31 & 34.4\% \\
\enddata
\tablenotetext{a}{All-Sky Automated Survey for SuperNovae \citep{shappee14,holoien17}}
\tablenotetext{b}{La Silla-Quest Low Redshift Survey \citep{baltay13}}
\tablenotetext{c}{Catalina Real Time Transit Survey \citep{djorgovski11}}
\tablenotetext{d}{Palomar Transient Factory \citep{law09} /Intermediate Palomar Transient Factory \citep{kulkarni13}}
\tablenotetext{e}{Pan-STARRS1 Medium Deep Survey \citep{kaiser10,scolnic18}}
\tablenotetext{f}{Kiso Supernova Survey \citep{morokuma14}}
\tablenotetext{g}{Mobile Astronomy System of TElescope Robots \citep{gorbovskoy13}}
\tablenotetext{h}{OGLE-IV Real-Time Transient Search \citep{wyrzykowski14}}
\tablenotetext{i}{Robotic Optical Transient Search Experiment III \citep{akerlof03}}
\tablenotetext{j}{Backyard Observatory Supernova Search \url{http://bosssupernova.com/}}
\tablenotetext{k}{CHilean Automatic Supernova sEarch \citep{pignata09}}
\tablenotetext{l}{T\'elescopes \`a Action Rapide pour les Objets Transitoires \citep{klotz08}}
%\tablenotetext{k}{Lick Observatory SN Search \citep{filippenko01}}
\tablenotetext{m}{THU-NAOC Transient Survey \citep{zhang15}}
%\tablenotetext{n}{Italian Supernovae Search Project \url{http://italiansupernovae.org/en/project/description.html}}
\tablenotetext{o}{\citet{CBET2943,nakano11,cox12,itagaki12,rich12,nishiyama12,yusa12,gagliano13,cortini13,kiyota13,kot13}}
\end{deluxetable}

==> v5.0 arXiv/Tables/Tab4.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{llclcc}
\tabletypesize{\scriptsize}
\tablecolumns{5}
\tablewidth{0pt}
\tablecaption{CSP-II Measurements of Host Galaxy Redshifts\label{tab:redshifts}}
\tablehead{
 & & & &  \multicolumn{2}{c}{lines\tablenotemark{c}}  \\
\colhead{SN} &
\colhead{Host Galaxy} &
\colhead{Instrument(s)\tablenotemark{a}} &
\colhead{$z_{Helio}$\tablenotemark{b}} &
\colhead{a} &
\colhead{e} 
%\colhead{Features Measured\tablenotemark{d}}
}
\startdata
ASASSN-14hu & ESO 058- G 012                   & 1 & $0.0216 \pm 0.0001$ & 1 & 5 \\ 
ASASSN-14jz & GALEXASC J184443.33-524819.2     &  1 & $0.0158 \pm 0.0001$ & \nodata & 8 \\
ASASSN-14kd & 2MASX J22532475+0447583          & 2 & $0.0242 \pm 0.0002$ & 1 & 3 \\
ASASSN-14lw & GALEXASC J010647.95-465904.1     &  2 & $0.0209 \pm 0.0001$ & \nodata & 3 \\
ASASSN-14me & ESO 113- G 047                   &   4 & $0.0178 \pm 0.0001$ & \nodata & 5  \\
ASASSN-15al & GALEXASC J045749.46-213526.3     &  1 & $0.0338 \pm 0.0001$ & 2 & 3 \\
ASASSN-15as & SDSS J093916.69+062551.1         &  1 & $0.0286 \pm 0.0001$ & \nodata & 3 \\
ASASSN-15bm & LCRS B150313.2-052600            &  1 & $0.0208 \pm 0.0003$ & 1 & 4 \\
ASASSN-15gr & ESO 366- G 015                   &  1 & $0.0243 \pm 0.0002$ & \nodata & 5 \\
ASASSN-15hx & GALEXASC J134316.80-313318.2     &  4 & $0.0083 \pm 0.0002$ & \nodata & 4 \\
CSS120325:123816-150632 & anonymous                        &  2 & $0.0972 \pm 0.0002$ & \nodata & 5 \\
CSS130215:033841+101827 (SN2013ad) & anonymous                        &  2 & $0.0363 \pm 0.0001$ & \nodata & 4 \\
CSS130303:105206-133424 & GALEXASC J105206.27-133420.2     &  1 & $0.0789 \pm 0.0004$ & \nodata & 1 \\
CSS130315:115252-185920 (SN2013as) & anonymous                        & 1 & $0.0685 \pm 0.0001$ & \nodata & 7 \\
CSS140126:120307-010132         &   SDSS J120306.76-010132.4 & 2 & $0.0772 \pm 0.0001$ & \nodata & 4 \\
CSS140218:095739+123318 & SDSS J095738.31+123308.5         & 2 & $0.0773 \pm 0.0002$ & \nodata & 1 \\
LSQ11bk  & anonymous                        &  2 & $0.0403 \pm 0.0001$ & \nodata & 5 \\
LSQ12ca  & 2MASX J05310364-1948063          &  4 & $0.0994 \pm 0.0003$ & \nodata & 3  \\
LSQ12agq & GALEXASC J101741.80-072452.2     &  3 & $0.0642 \pm 0.0001$ & \nodata & 6 \\
LSQ12aor & GALEXASC J105517.85-141757.2     &  3 & $0.0934 \pm 0.0001$ & \nodata & 8 \\
LSQ12cdl & GALEXASC J125339.85-183025.6     &  2 & $0.1081 \pm 0.0001$ & \nodata & 6 \\
LSQ12fuk & GALEXASC J045815.88-161800.7     & 1 & $0.0206 \pm 0.0002$ & \nodata & 4 \\
LSQ12gef & 2MASX J01403375+1830406          & 1 & $0.0642 \pm 0.0004$ & 6 & 3 \\
LSQ12gln & GALEXASC J052259.58-332755.3     & 3 & $0.1021 \pm 0.0001$ & \nodata & 8 \\
LSQ12gpw & 2MASX J03125885-1142402          &  1 & $0.0506 \pm 0.0002$ & 1 & 4 \\
LSQ12gzm & GALEXASC J024043.58-344425.0     &  4 & $0.1001 \pm 0.0002$ & \nodata & 5  \\
LSQ12hjm & 2MASX J03102844-1629333          & 1 & $0.0714 \pm 0.0002$ & 2 & 6 \\
LSQ12hno & GALEXASC J034243.43-024007.7     &  1 & $0.0473 \pm 0.0001$ & \nodata & 7 \\
LSQ12hvj & GALEXASC J110738.65-294235.5     & 1 & $0.0713 \pm 0.0001$ & \nodata & 4 \\
LSQ12hzj & 2MASX J09591230-0900095          &  2,4 & $0.0334 \pm 0.0002$ & 4 & \nodata \\
LSQ13lq & SDSS J134410.77+030345.3         & 1 & $0.0757 \pm 0.0002$ & \nodata & 4 \\
LSQ13pf & LCRS B134534.3-112338            & 2 & $0.0861 \pm 0.0001$ & 1 & 3 \\
LSQ13vy  & 2MASX J16065563+0300046          &  1 & $0.0418 \pm 0.0004$ & 4 & 4 \\
%LSQ13aiz (SN2013cs) & ESO 576- G 017                   &  4 & $0.0930 \pm 0.0002$ & \nodata & 5   \\
LSQ13dcy & LCSB S0801P                      &  1,4 & $0.0801 \pm 0.0003$ & 7 & \nodata \\
LSQ13dhj & GALEXMSC J021234.60-372019.1     &  1,4 & $0.0935 \pm 0.0001$ & \nodata & 5 \\
%LSQ13dkp & 2MASX J03101094-3638017          &  1 & $0.0692 \pm 0.0002$ & 6 & \nodata \\
LSQ13dpm & GALEXASC J102908.61-170654.2     & 1 & $0.0509 \pm 0.0003$ & \nodata & 4 \\
LSQ13dqh & anonymous                        &  2 & $0.1038 \pm 0.0001$ & \nodata & 4 \\
LSQ13dsm & APMUKS(BJ) B033105.19-262232.9   &  1 & $0.0424 \pm 0.0002$ & \nodata & 5 \\
LSQ14ba & GALEXASC J110123.17-153706.2     & 1 & $0.0776 \pm 0.0001$ & \nodata & 4 \\
LSQ14ie  & anonymous                        & 1 & $0.0896 \pm 0.0001$ & \nodata & 5 \\
LSQ14wp & SDSS J101405.83+064032.5         &  2 & $0.0695 \pm 0.0001$ & \nodata & 4 \\
LSQ14age & GALEXASC J132408.58-132629.0     &  1 & $0.0806 \pm 0.0003$ & \nodata & 5 \\
LSQ14ahc & 2MASX J13434760-3254381          & 2 & $0.0509 \pm 0.0001$ & \nodata & 3 \\
LSQ14ahm & GALEXASC J114122.65-122354.9     & 1 & $0.0498 \pm 0.0001$ & \nodata & 4 \\
LSQ14bbv & 2MASS J19593264-5659334          &  1 & $0.0588 \pm 0.0006$ & 7 & \nodata \\
LSQ14bjj & APMUKS(BJ) B141811.91-050120.8   & 1 & $0.0812 \pm 0.0001$ & \nodata & 7 \\
LSQ14fms & 2MASX J00145929-5112380          & 1 & $0.078 \pm 0.001$  & 3 & 2 \\
LSQ14gfn & 2MASX J03283205-0412113          &  2 & $0.1217 \pm 0.0004$ & 6 & \nodata \\ 
LSQ14gov & GALEXMSC J040601.67-160139.7     & 1 & $0.0896 \pm 0.0002$ & \nodata & 5 \\
LSQ15aae & 2MASX J16301506+0555514          & 1 & $0.0516 \pm 0.0001$ & 1 & 2 \\
LSQ15aja & SDSS J170308.90+122741.5     &  2 & $0.0700 \pm 0.0001$ & \nodata & 4 \\
MASTER OT J030559.89+043238.2 & SDSS J030559.63+043246.0         &  1 & $0.0282 \pm 0.0009$ & \nodata & 3 \\
%MLS140102:120307-010132 & SDSS J120306.76-010132.4         &  2 & $0.0772 \pm 0.0001$ & \nodata & 4 \\
OGLE-2013-SN-015 & 2MASX J02022241-6544090          &  1,4 & $0.0890 \pm 0.0002$ & 4 & \nodata \\
OGLE-2013-SN-109 & 2MASX J01460987-6727579          & 1,4 & $0.0868 \pm 0.0001$ & \nodata & 5 \\
OGLE-2013-SN-118 & 2MASX J05144615-6650292          &  1 & $0.0750 \pm 0.0002$ & \nodata & 5 \\
OGLE-2013-SN-123 & 2MASX J05583036-6333386          & 1 & $0.0614 \pm 0.0002$ & 9 & \nodata \\
OGLE-2013-SN-126 & anonymous                        &  2 & $0.0597 \pm 0.0002$ & \nodata & 3 \\
OGLE-2013-SN-148 & 2MASX J06380745-7543288          & 1 & $0.0404 \pm 0.0002$ & \nodata & 6 \\
OGLE-2014-SN-021 & anonymous                        &  3 & $0.0422 \pm 0.0002$ & \nodata & 6 \\
OGLE-2014-SN-107 & APMUKS(BJ) B004021.02-650219.5   & 1 & $0.0664 \pm 0.0001$ & \nodata & 3 \\
OGLE-2014-SN-141 & 2MASX J05371898-7543157          & 1 & $0.0625 \pm 0.0002$ & 1 & 8 \\ 
PS15sv   & GALEXASC J161311.68+013532.2     &  1 & $0.0333 \pm 0.0003$ & \nodata & 5 \\ 
PTF11ppn & 2MASX J21352164+2656051          & 1 & $0.0673 \pm 0.0002$ & 8 & \nodata \\
iPTF13anh & SDSS J130650.44+153432.7         &  2 & $0.0614 \pm 0.0001$ & \nodata & 6 \\
iPTF13dwl & GALEXASC J211648.97+120052.8     & 1 & $0.0875 \pm 0.0002$ & \nodata & 6 \\
iPTF13efe & SDSS J084339.26+161037.5         & 2 & $0.0751 \pm 0.0001$ & \nodata & 4 \\
iPTF14uo & GALEXASC J131857.37+094244.0     & 2 & $0.0913 \pm 0.0001$ & \nodata & 7 \\
ROTSE3 J123935.1+163512 & IC 0803 NED01 (SN2012G)      &  4 & $0.0258 \pm 0.0002$ & \nodata & 5  \\
SMTJ03253351-5344190 & anonymous                        &  3 & $0.0592 \pm 0.0002$ & \nodata & 5 \\
SNhunt161 (SN2012hl)   & CSS J005017.69+243154.4  & 5 & $0.0332 \pm 0.0002$ & \nodata & 6  \\
\enddata
%SN2014dk & 1 & $0.0319 \pm 0.0009$ & 4 & Ca II H,K, G-band, 4710\\
%CSS140501:170414+174839 & 1 & $0.0798 \pm 0.0003$ & 5 & [N II]6548,6583, H$\alpha$, [S II]6717,6731\\
%LSQ14fmg & 1 & $0.0661 \pm 0.0003$ & 4 & [N II]6548,6583, H$\alpha$, [S II]6717\\
%LSQ15adm & 1 & $0.0723 \pm 0.0003$ & 6 & [O II]3727, [N II]]6548,6583, H$\alpha$, [S II]6717,6731\\
%LSQ15agh & 1 & $0.0600 \pm 0.0002$ & 7 & Ca II H,K, G-bsnd, H$\alpha$, [NII]6583, [SII]6717,6731\\
\tablenotetext{a} {1: du Pont+WFCCD, 2: Magellan Baade+IMACS, 3: Magellan Clay+LDSS3, 4: VLT+MUSE, 5: Calar Alto~3.5~m+PMAS/PPak}
\tablenotetext{b} {The heliocentric redshift measurement was derived from the equivalent-width-weighted average of 
the features listed in final column.  A minimum error of 0.0001 is adopted from instrumental resolution considerations.}
\tablenotetext{c} {Number of absorption (a) and emission (e) lines used to measure the redshift.  Wavelengths of the
features used to calculate the redshift are taken from Table~II of \citet{sandage78}.}
\end{deluxetable*}
\end{longrotatetable}

==> v5.0 arXiv/Tables/Tab5.tex <==
\begin{deluxetable} {ccc}
\tabletypesize{\scriptsize}
\tablecolumns{3}
\tablewidth{0pt}
\tablecaption{Optical Photometric Reduction Terms: SITe3 vs. e2V\label{tab:ec_ct}}
\tablehead{
\colhead{Filter} &
\colhead{Swope+SITe3}   &
\colhead{Swope+e2V}
}
\startdata
\multicolumn{3}{c}{Extinction Coefficients\tablenotemark{a}} \\
$u$ & \phn0.511 $\pm$ 0.057 &  0.509 $\pm$ 0.060 \\
$B$ & \phn0.242 $\pm$ 0.022 &  0.233 $\pm$ 0.027 \\
$g$ & \phn0.191 $\pm$ 0.021 & 0.186 $\pm$ 0.027 \\
$V$ & \phn0.144 $\pm$ 0.018 & 0.135 $\pm$ 0.026 \\
$r$ & \phn0.103 $\pm$ 0.019 & 0.094 $\pm$ 0.022 \\
$i$ & \phn0.059 $\pm$ 0.020 & 0.057 $\pm$ 0.020 \\
\hline
\multicolumn{3}{c}{Color Terms\tablenotemark{b}} \\
$u$ & \phn0.046 $\pm$ 0.017 & \phn0.030 $\pm$ 0.020  \\
$B$ & \phn0.061 $\pm$ 0.012 & \phn0.091 $\pm$ 0.015 \\
$g$ & $-$0.014 $\pm$ 0.011 &  $-$0.005 $\pm$ 0.014 \\
$V$ & $-$0.058 $\pm$ 0.011 & $-$0.062 $\pm$ 0.015 \\
$r$ & $-$0.016 $\pm$ 0.015 & $-$0.001 $\pm$ 0.022 \\
$i$ & $-$0.002 $\pm$ 0.015 & \phn0.021 $\pm$ 0.018 \\
\enddata
\tablenotetext{a}{Measured in magnitudes per airmass.  
All unncertainties in this table are the ``standard deviations 
of the distributions,'' not the standard deviations of the means.}
\tablenotetext{b}{See equations~\ref{eq:u_inst}--\ref{eq:V_inst}
for which standard colors are used in combination with these coefficients 
to obtain the color correction terms for the optical photometry.}
\end{deluxetable}


==> v5.0 arXiv/Tables/Tab6.tex <==
\begin{deluxetable} {ccc}
\tabletypesize{\scriptsize}
\tablecolumns{3}
\tablewidth{0pt}
\tablecaption{NIR Photometric Reduction Terms \label{tab:nir_ec_ct}}
\tablehead{
\colhead{Filter} &
\colhead{du~Pont~+~RetroCam}   &
\colhead{Baade~+~FourStar}
}
\startdata
 & \multicolumn{2}{c}{Extinction Coefficients\tablenotemark{a}} \\
$Y$ & \phn0.069 $\pm$ 0.006 &  \ldots \\
$J$ & \phn0.101 $\pm$ 0.006 &  \ldots \\
$H$ & \phn0.056 $\pm$ 0.007 & \ldots \\
\hline
 & \multicolumn{2}{c}{Color Terms\tablenotemark{b}} \\
$Y$ & \phn0.000 & \phn0.106 \\
$J$ & \phn0.019 &  \phn0.001 \\
$H$ & $-$0.039 & $-$0.040 \\
\enddata
\tablenotetext{a}{Measured in magnitudes per airmass.  
Unncertainties in the extinction coefficients are the ``standard deviations 
of the distributions,'' not the standard deviations of the means.}
\tablenotetext{b}{See equations~\ref{eq:y_inst}--\ref{eq:h_inst}
for which standard colors are used in combination with these coefficients 
to obtain the color correction terms for the NIR photometry. The
color terms in this table are estimated from synthetic photometry of \citet{castelli03}
stellar atmosphere models.  The extinction coefficients measured for the
du~Pont~+~RetroCam were assumed for Baade~+~FourStar.}
\end{deluxetable}

